HexaLab.net: an online viewer for hexahedral meshes

We introduce HexaLab: a WebGL application for real time visualization, exploration and assessment of hexahedral meshes. HexaLab can be used by simply opening www.hexalab.net. Our visualization tool targets both users and scholars. Practitioners who employ hexmeshes for Finite Element Analysis, can readily check mesh quality and assess its usability for simulation. Researchers involved in mesh generation may use HexaLab to perform a detailed analysis of the mesh structure, isolating weak points and testing new solutions to improve on the state of the art and generate high quality images. To this end, we support a wide variety of visualization and volume inspection tools. Our system offers also immediate access to a repository containing all the publicly available meshes produced with the most recent techniques for hexmesh generation. We believe HexaLab, providing a common tool for visualizing, assessing and distributing results, will push forward the recent strive for replicability in our scientific community.

==> result.tex <==
% !TEX root =  main_hexalab.tex

% Qui si descrive l'applicazione in pratica
% descrivendo in dettaglio una sessione e facendo vedere le varie funzionalita
% Si dovrebbe riportare anche se possibile eventuali feedback

%\section{Results}

%\begin{figure*}[h]
%\centering
%\fbox{
%\includegraphics[width =0.7\linewidth]{images/missing.png}
%}
%\caption{The main application window}
%\label{app}
%\end{figure*}

%Figure \ref{app} shows the main web application window (www.hexalab.it). The main portion of the page is dedicated to the rendering of the mesh. The viewing position and angle can be controlled by interacting with the canvas. By dragging the left mouse button it is possible to rotate around the focus point, which by default is centered on the mesh, and by dragging the right mouse button it is possible to move the focus point. Finally, by scrolling the mouse wheel it is possible to zoom in and out.

%The sidebar to the left is the only other element in the page and it contains all the remaining user interface controls. The topmost toolbar exposes the basic application features.


%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/toolbar.png}
%\caption{The main toolbar functionalities: Import a mesh; Reset the viewing position and angle; Visualize the histogram of element's quality; Import a custom settings file; Save the current settings configuration to a local file; Take a snapshot of the canvas and save it locally; Link to the GitHub project page. }
%\label{toolbar}
%\end{figure}

%Their respective functionality are:
%\begin{itemize}[noitemsep,topsep=0pt]
%    \item Import a mesh local to the client
 %   \item Reset the viewing position and angle
 %   \item Visualize the mesh quality on an histogram
%    \item Import a custom settings file
%    \item Save the current settings configuration to a local file
 %   \item Take a snapshot of the canvas and save it locally
 %   \item Link to the GitHub project page
%\end{itemize}

%As previously mentioned, currently the only supported format by the importer is the .mesh format. The default viewing position is determined depending on the mesh position and bounding size, with the aim to create a normalized viewpoint that produces similar results for all mesh inputs. The mesh quality histogram displays the distribution of the selected quality estimator. The colors used are the same as those picked for the rendering.

%It is possible to swap the plot axis and to save the figure on a local file through the local toolbar. 

%\Hexalab can export setting configurations to be reused later. The configurations are not tied to the mesh and include many parameters, from the viewing position to the filters settings. This allows users, for example, to adopt a standard point of view and settings configuration to view a set of meshes, or to share a mesh file along with its settings file to recreate the same visual result for both users.


%Below the toolbar are the filters configurations, one after the other.

%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/filters.png}
%\caption{The filters panels.}
%\label{filters}
%\end{figure}

%There are only two filters currently implemented into the application:
%\begin{itemize}[noitemsep,topsep=0pt]
%   \item A position-based filter, acting like a culling plane
%    \item A quality-based filter
%\end{itemize}
%The plane panel allows to control the first filter by changing the normal vector and the offset from the mesh center of the plane. The normal is controlled by three separate text fields and the offset is controlled by both a text field and a sliding bar. The buttons offer additional control over the normal vector, allowing to quickly snap its the x, y or z component to the respective orthonormal axis, to flip it and to set it in the same direction as the viewer. 

%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/plane2.png}
%\caption{A plane-filtered mesh rendering.}
%\label{plane}
%\end{figure}

%The second panel allows the control of the quality filter by changing the method used to estimate the quality and the visualized range. The only method currently implemented is the Scaled Jacobian estimation.  The range of quality values to be visualized is controlled by both a sliding bar and two text fields. Additionally, the button allows to quickly flip the selected range.

%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/quality2.png}
%\caption{A quality-filtered mesh rendering with quality display turned on.}
%\label{quality}
%\end{figure}

%The next panel contains controls concerning rendering and visualization modes. 

%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/rendering.png}
%\caption{The rendering settings panel.}
%\label{rendering}
%\end{figure}

%The color of the mesh surface is controlled by a color picker. The transparency of the filtered portion of the mesh surface and that of the singularity edges indicators are regulated through two sliding bars. A checkbox allows to enable or disable the mode where instead of using surface color, each hexa color is mapped to a value depending on its quality. Another checkbox enables or disables ambient occlusion. Finally, it is possible to pick which color mapping to use to display quality through a select box. This change will also affect the colors used to plot the quality distribution histogram.

%\begin{figure}[h]
%\centering
%\includegraphics[width =0.9\linewidth]{images/sing.png}
%\caption{An example of displaying all the singularity edges of a mesh.}
%\label{sing}
%\end{figure}

%We also included a simple texbox panel  containing the application logging output, to give additional information to the user and to give a small partial history of the operations executed by the backend. Each main computational pass performed outputs a descriptive line along with the time occupied.
%Events like canvas resizes are logged, too.


